Toward Scalable, Flexible Scene Flow for Point Clouds

Scene flow estimation is the task of describing 3D motion between temporally successive observations. This thesis aims to build the foundation for building scene flow estimators with two important properties: they are scalable, i.e. they improve with access to more data and computation, and they are flexible, i.e. they work out-of-the-box in a variety of domains and on a variety of motion patterns without requiring significant hyperparameter tuning. In this dissertation we present several concrete contributions towards this. In Chapter 1 we contextualize scene flow and its prior methods. In Chapter 2 we present a blueprint to build and scale feedforward scene flow estimators without requiring expensive human annotations via large scale distillation from pseudolabels provided by strong unsupervised test-time optimization methods. In Chapter 3 we introduce a benchmark to better measure estimate quality across diverse object types, better bringing into focus what we care about and expect from scene flow estimators, and use this benchmark to host a public challenge that produced significant progress. In Chapter 4 we present a state-of-the-art unsupervised scene flow estimator that introduces a new, full sequence problem formulation and exhibits great promise in adjacent domains like 3D point tracking. Finally, in Chapter 5 I philosophize about what's next for scene flow and its potential future broader impacts.

==> PackagesLoadedbyTemplate.tex <==
% University of Pennsylvania Ph.D. Dissertation LaTeX Template packages

upennstyle.sty loads the following packages
\begin{itemize}
\item amscd
\item amsfonts
\item amsmath
\item amssymb
\item amsthm
\item appendix
\item array
\item babel
\item blindtext
\item booktabs
\item calc
\item caption
\item csquotes
\item float
\item fontenc
\item geometry 
\item graphicx
\item hyperref
\item multirow
\item parskip
\item pdflscape
\item setspace
\item tabularx
\item titlesec
\item tocloft
\item verbatim
\end{itemize}

sampledissertation.tex loads the following packages
\begin{itemize}
\item upennstyle
\item natbib
\end{itemize}

==> eulerflow/abstract_hardstyle.tex <==
%We present a step function unlock in unsupervised scene flow capabilities. 
We reframe scene flow as the task of estimating a continuous space-time ODE that describes motion for an entire observation sequence, represented with a neural prior. Our method, \emph{\ourmethod{}}, optimizes this neural prior estimate against several multi-observation reconstruction objectives, enabling high quality scene flow estimation via pure self-supervision on real-world data. \ourmethod{} works out-of-the-box without tuning across multiple domains, including large-scale autonomous driving scenes and dynamic tabletop settings. Remarkably, \ourmethod{} produces high quality flow estimates on small, fast moving objects like birds and tennis balls, and exhibits emergent 3D point tracking behavior by solving its estimated ODE over long-time horizons. On the Argoverse 2 2024 Scene Flow Challenge, \ourmethod{} outperforms \emph{all} prior art, surpassing the next-best \emph{unsupervised} method by more than $2.5\times$, and even exceeding the next-best \emph{supervised} method by over 10\%.


%performs well in diverse domains --- applied to the autonomous vehicle domain, \textbf{\ourmethod{} outperforms \emph{all} prior art, unsupervised or supervised}, on the Argoverse~2 2024 Scene Flow Challenge leaderboard, as well as other common real-world benchmarks; applied to dynamic tabletop domain, \ourmethod{} produces good quality scene flow out-of-the-box without tuning. 

%Notably, \ourmethod{} is capable of providing high quality motion descriptions for small objects, including those outside any labeled object taxonomy, making good on the promise of scene flow as a strong signal for open-world object detection. \ourmethod{} produces good quality scene flow out-of-the-box on real-world data in multiple domains, including dynamic tabletop settings, and solving the PDE for long time horizons exhibits emergent capabilities such as basic 3D point tracking behavior.

%We present a step-function unlock in unsupervised capabilities. We reframe scene flow as the problem of estimating a continuous space and time PDE that describes positional change for an entire observation sequence, represented by a neural prior. Our resulting unsupervised method, \emph{\ourmethod{}}, performs well qualitatively and qualitatively in diverse domains --- \ourmethod{} outperforms \emph{all} prior art, unsupervised or supervised, on the Argoverse~2 2024 Scene Flow Challenge leaderboard, as well as other common real-world benchmarks, and with no changes can produce high quality flow estimates in the tabletp.

%Contemporary unsupervised scene flow methods typically only use two consecutive frames to estimate per-point 3D motion. However, accurately describing object motion from two frames is particularly challenging and can lead to inconsistent long-term trajectories. In contrast, recent state-of-the-art supervised scene flow methods demonstrate that multi-sweep aggregation yields more accurate motion estimates. We argue that unsupervised scene flow estimation should be similarly recast to take advantage of all frames in a sequence. To this end, we propose \ourmethod{}, an unsupervised approach for fitting a continuous space-time partial differential equation (PDE) to describe per-point motion across an entire sequence. We demonstrate that \ourmethod{} produces high quality scene flow on real-world data across multiple domains, including large-scale autonomous driving scenes and dynamic tabletop settings. Notably, \ourmethod{} provides high quality motion descriptions for small objects, including open-world categories like {\tt bird} and {\tt tennis ball}. Lastly, we find that our sequence-level optimization facilitates emergent 3D point tracking without explicit supervision. Our proposed approach significantly reduces mean Dynamic EPE by 2.5 $\times$, resoundingly outperforming {\em all} prior unsupervised methods on the Argoverse 2 Scene Flow benchmark. Moreover, \ourmethod{} beats the prior {\em supervised} state-of-the-art by 10.3\%!

==> eulerflow/tex_figures/bird_one_row.tex <==
\begin{figure}[htb]
\centering
% First row
\begin{subfigure}[b]{0.16\textwidth}
    \centering
    \includegraphics[width=\textwidth]{screenshot_figures/flying_bird/000000_test_gigachad_nsf_depth18_flattened_subsequence_length_150_cropped.png}
    \caption{\ourmethod{}}
    \figlabel{flyingbirdgigachad}
\end{subfigure}%
\begin{subfigure}[b]{0.16\textwidth}
    \centering
    \includegraphics[width=\textwidth]{screenshot_figures/flying_bird/000000_test_fast_nsf_flow_feather_subsequence_length_150_cropped.png}
    \caption{Fast NSF}
    \figlabel{flyingbirdfastnsf}
\end{subfigure}%
\begin{subfigure}[b]{0.16\textwidth}
    \centering
    \includegraphics[width=\textwidth]{screenshot_figures/flying_bird/000000_test_bucketed_nsfp_distillation_5x_out_subsequence_length_150_cropped.png}
    \caption{ZeroFlow 5x}
    \figlabel{flyingbirdzeroflow}
\end{subfigure}
\begin{subfigure}[b]{0.16\textwidth}
    \centering
    \includegraphics[width=\textwidth]{screenshot_figures/flying_bird/000000_test_liu_flow_feather_subsequence_length_150_cropped.png}
    \caption{\citeauthor{liu2024selfsupervisedmultiframeneuralscene}}
    \figlabel{flyingbirdliuetal}
\end{subfigure}%
\begin{subfigure}[b]{0.16\textwidth}
    \centering
    \includegraphics[width=\textwidth]{screenshot_figures/flying_bird/000000_test_nsfp_flow_feather_subsequence_length_150_cropped.png}
    \caption{NSFP}
    \figlabel{flyingbirdnsfp}
\end{subfigure}%
\begin{subfigure}[b]{0.16\textwidth}
    \centering
    \includegraphics[width=\textwidth]{screenshot_figures/flying_bird/000000_test_sceneflow_feather_subsequence_length_150_cropped.png}
    \caption{Ground Truth}
    \figlabel{flyingbirdgt}
\end{subfigure}
%\texttt{5f016e44-0f38-3837-9111-58ec18d1a5e6}
\caption{Qualitative visualization of \ourmethod{} compared to prior art for the same scene as \figref{teasersceneflow} and \figref{birdtrajectory}. \ourmethod{} is able to cleanly extract the bird's trajectory; however, all other methods except \citeauthor{liu2024selfsupervisedmultiframeneuralscene} fail to recognize this motion, and \citeauthor{liu2024selfsupervisedmultiframeneuralscene}'s flow is non-smooth and marred by severe scene artifacts. Note that the bird is outside the labeled object taxonomy, and so its motion is not labeled in the ground truth (\figref{flyingbirdgt}).\vspace{-1em}}
\figlabel{flyingbird}
\end{figure}

==> eulerflow/tex_figures/two_frame_vs_full_sequence_4x3.tex <==

\begin{figure}[phtb]
\centering
% First row: Two Frame figures
\begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{screenshot_figures/walking_ped/000043_test_gigachad_nsf_depth18_flattened_subsequence_length_2.png}
    \caption{\ourmethod{} (Two Frame)}
    \figlabel{flyingbirdgigachad_twoframe}
\end{subfigure}%
\begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{screenshot_figures/walking_ped/000043_test_fast_nsf_flow_feather_subsequence_length_2.png}
    \caption{Fast NSF (Two Frame)}
    \figlabel{flyingbirdfastnsf_twoframe}
\end{subfigure}%
\begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{screenshot_figures/walking_ped/000043_test_bucketed_nsfp_distillation_5x_out_subsequence_length_2.png}
    \caption{ZeroFlow 5x (Two Frame)}
    \figlabel{flyingbirdzeroflow_twoframe}
\end{subfigure}

% Second row: Two Frame figures continued
\begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{screenshot_figures/walking_ped/000043_test_liu_flow_feather_subsequence_length_2.png}
    \caption{\citeauthor{liu2024selfsupervisedmultiframeneuralscene} (Two Frame)}
    \figlabel{flyingbirdliuetal_twoframe}
\end{subfigure}%
\begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{screenshot_figures/walking_ped/000043_test_nsfp_flow_feather_subsequence_length_2.png}
    \caption{NSFP (Two Frame)}
    \figlabel{flyingbirdnsfp_twoframe}
\end{subfigure}%
\begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{screenshot_figures/walking_ped/000043_test_sceneflow_feather_subsequence_length_2.png}
    \caption{Ground Truth (Two Frame)}
    \figlabel{flyingbirdgroundtruth_twoframe}
\end{subfigure}

% Third row: Full Sequence figures
\begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{screenshot_figures/walking_ped/000000_test_gigachad_nsf_depth18_flattened_subsequence_length_150.png}
    \caption{\ourmethod{} (Full Sequence)}
    \figlabel{flyingbirdgigachad_fullsequence}
\end{subfigure}%
\begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{screenshot_figures/walking_ped/000000_test_fast_nsf_flow_feather_subsequence_length_150.png}
    \caption{Fast NSF (Full Sequence)}
    \figlabel{flyingbirdfastnsf_fullsequence}
\end{subfigure}%
\begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{screenshot_figures/walking_ped/000000_test_bucketed_nsfp_distillation_5x_out_subsequence_length_150.png}
    \caption{ZeroFlow 5x (Full Sequence)}
    \figlabel{flyingbirdzeroflow_fullsequence}
\end{subfigure}

% Fourth row: Full Sequence figures continued
\begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{screenshot_figures/walking_ped/000000_test_liu_flow_feather_subsequence_length_150.png}
    \caption{\citeauthor{liu2024selfsupervisedmultiframeneuralscene} (Full Sequence)}
    \figlabel{flyingbirdliuetal_fullsequence}
\end{subfigure}%
\begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{screenshot_figures/walking_ped/000000_test_nsfp_flow_feather_subsequence_length_150.png}
    \caption{NSFP (Full Sequence)}
    \figlabel{flyingbirdnsfp_fullsequence}
\end{subfigure}%
\begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{screenshot_figures/walking_ped/000000_test_sceneflow_feather_subsequence_length_150.png}
    \caption{Ground Truth (Full Sequence)}
    \figlabel{flyingbirdgroundtruth_fullsequence}
\end{subfigure}

\caption{\figrefs{flyingbirdgigachad_twoframe}{flyingbirdgroundtruth_twoframe} show a typical two frame scene flow visualization of \ourmethod{} and several baseline methods, as commonly found in the scene flow literature. This scene features several pedestrians walking in front of a car stopped at a stop light near the ego vehicle, enabling unusually dense pedestrian observations and thus providing enough structure for baseline method to seemingly work. In this two frame paradigm, it is difficult to distinguish method quality, even upon careful inspection. By comparison, \figrefs{flyingbirdgigachad_fullsequence}{flyingbirdgroundtruth_fullsequence} show the full accumulated sequence, enabling a clearer qualitative understanding of flow quality and scene artifacts between methods.}
\figlabel{walkingpeds}
\end{figure}


==> overview_old.tex <==
\section{A (brief, opinionated) history of why motion description has become relevant}

Computer Vision as a field aims to understand the world. To turn this lofty ideal into a concrete goal, researchers invented problems like image classification or object detection and split off to try to make progress, along the way setting up benchmarks like ImageNet or COCO to measure this progress. These problems were largely formulated atop still images captured with a digital camera --- this kind of data was most readily available, and these problems were ``hard enough'' without adding in multiple frames to process. As a result, outside of problem formulations with immediate applications (e.g.\ optical flow for video compression), motion description was relatively unstudied at the outset.

Via a concerted effort, the computer vision community has produced standard recipes for training good quality deep learning systems on these single frame problems~\citep{alexnet, dinov2}. These recipes lean on a combination of data scale and clever unsupervised pretraining objectives~\citep{dinov2} --- training on larger, more diverse datasets produces better quality methods, and unsupervised pretraining objectives enable networks to be trained on internet scale datasets without requiring expensive and laborious human supervision. For images, these recipes have produced image foundation models that can competently solve many of our invented single image problems. For 3D data like lidar point clouds, the same general recipes have been successfully applied to analogous 3D problems~\citep{voxelnet, yan2018second, pointpillars}, although they do not benefit from availability of internet scale data.

This success of single frame methods has spawned \emph{Detect then Track}-style robotics control loops. In each iteration of the loop, the agent takes in the latest sensor reading, runs a single frame vision method to get current observation, runs a state estimator to integrate the that output with prior observations, runs a predictor to estimate the future trajectory of any moving objects, and then emits an action accordingly. This approach broadly works fine in structured domains like Autonomous Vehicles (AVs) where control is well understood; it's easy to avoid static structure with purely geometric techniques on lidar observations, and almost all non-ego moving objects are from known classes (cars, pedestrians, bicyclists), so a good single frame object detection and careful tuning of the full stack can produce a fairly competent driving system.

However, this paradigm fails when it encounters objects from the ``long tail'', i.e.\ objects outside of its detector's known taxonomy. Things like debris falling from the back of a truck or a tree falling in the road are unknown to a typical detector even on modern AV datasets. Even if you account for these specific scenarios, enough deployments in the real world will inevitably produce an encounter with an unknown moving object that the AV needs to avoid but its detector fails to detect. And this is not just for Autonomous Vehicles; other domains like indoor service robots consistently feature foreign moving objects that a robot has to interact with or potentially avoid. Fundamentally, these failures stem from the fact that \emph{Detect then Track} is the wrong paradigm to try to reason about arbitrary moving objects; handling this requires methods that understand motion via geometric motion cues without first requiring object detection.

This need has spawned renewed interest in motion description, with problems like point tracking, optical flow, and scene flow seeing renewed interest over the last several years. In this work, we discuss motion description is hard and what I have done to contribute to their advancement.


\section{What exactly is ``motion description'' and why is it hard?}

In the same way that ``object description'' encompasses several related problems like classification, object detection, semantic segmentation, or panoptic segmentation, ``motion description'' encompasses several related problems like point tracking and scene flow. At their core, these problems are simply different ways of expressing how a particular point on an object moves over time, but each problem formalism expects inputs and outputs to be expressed slightly differently. Unfortunately, none of these formulations are trivially self-supervised, and we have yet to clearly crack the code on the right pretraining objectives to scale them up like we have with object description problems.

\subsection{What is Optical Flow and why is it hard?}

Optical Flow is classically formulated as the problem of estimating per-pixel image space motion vectors describing how an image at $t$ warps to form the image at $t+1$~\citep{gibson1950, gibson1966, gibson1977, HORN1981185}; \figref{perceiver_sintel_example} provides an example input-output pair for scene flow.

\begin{figure}[htb!]
  \centering
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{intro_figures/sintel_input_1.png}
    \caption{$t$ input image}
    \label{fig:sintel_input_1}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{intro_figures/sintel_input_2.png}
    \caption{$t+1$ input image}
    \label{fig:sintel_input_2}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.32\textwidth}
    \centering
    \includegraphics[width=\textwidth]{intro_figures/sintel_optical_flow.png}
    \caption{Optical Flow}
    \label{fig:sintel_optical_flow}
  \end{subfigure}
  \caption{An example of optical flow on the Sintel synthetic dataset \citep{sintel}. \figref{sintel_optical_flow} describes the image space motion of \figref{sintel_input_1} (at $t$) as it moves into the view of \figref{sintel_input_2} (at $t+1$); the color of each pixel describes flow direction, while intensity describes its magnitude, with white being $\vec{0}$.}
  \figlabel{perceiver_sintel_example}
\end{figure}

Optical flow estimates contain the addition of two separate pieces of information: how the camera is moving relative to the static background, as well as how other objects in the scene are moving. As an example of this, in \figref{perceiver_sintel_example} the camera is panning to the right (causing the background rock face to appear to be moving to the left), while the dragon moves to the right and the person is standing up from a crouched position.

Historically, researchers tackled optical flow with classical dense stereo correspondence algorithms \citep{scharstein2002taxonomy} combined with optimization techniques \citep{brox2010large, sundaram2010dense}, but more recent methods learn optical flow  from supervision \citep{dosovitskiy2015flownet, ilg2017flownet, li2022rigidflow}, attempting to imitate the deep learning recipes that worked well for structure understanding.

Scene flow is hard because researchers must either hand design optimization approaches (which improve with researcher effort, not just from access to more data and compute), or they must obtain supervision. Supervision for optical flow is extremely difficult to obtain --- it requires dense, pixel perfect motion labels that precisely capture both camera motion as well as any non-ego scene motion. Consequently, almost all learned methods rely upon synthetic datasets such as FlyingThings~\citep{flyingthings}, a dataset of random objects randomly moving, or Sintel~\citep{sintel} / Spring~\citep{spring}, datasets constructed from scenes from open source 3D animated movies by the same name, with only a meager amount of real-world data available from sources like the KITTI dataset~\citep{kittisceneflow1, kittisceneflow2}. 


% TODO SAY SOMETHING ABOUT DEEP LEARNING

% TODO LOOK AT SEA-FLOW RELATED WORK https://arxiv.org/pdf/2405.14793

% TODO TALK ABOUT DATASETS
% - FlyingThings~\citep{flyingthings}
% - Sintel~\citep{}
% - Spring

\subsection{What is Scene Flow and why is it hard?}

Scene Flow is a generalization of optical flow into 3D, where vectors describe motion in some metric space. Scene flow was first formulated with stereo image inputs~\citep{vedula1999}, which in the literature is considered equivalent to RGB+Depth inputs due to the ability to estimate depth from stereo disparities~\citep{pons2007multi}. \cite{dewan2016rigid} generalized scene flow to arbitrary point clouds, removing the regular grid structure found in images and making approaches suitable for use on time-of-flight sensors like lidar that produce an unordered set of 3D points. 

Scene flow can be solved by piggybacking off of optical flow, and lifting this result into 3D~\citep{opticalexpansion}, but most modern methods  either perform optimization against hand designed surrogate objectives over 3D flow volume~\citep{nsfp,fastnsf,liu2024selfsupervisedmultiframeneuralscene} or learn to estimate flow from supervision~\citep{flownet3d, li2022rigidflow, scalablesceneflow, zhang2024deflow}.

Like with optical flow, scene flow is hard because methods rely on human engineered surrogate objectives or on expensive supervision. Interestingly, unlike optical flow which requires laborious, pixel perfect image labeling, the 3D nature of scene flow makes it expensive but tractable to label real-world data. Ego-motion can be straightforwardly be solved for with global alignment approaches, allowing human labelers to only focus on labeling the motion of other moving objects. Consequently, scene flow is less dependent upon strictly synthetic data, which often has unrealistic motion and scan patterns~\citep{chodosh2023}. In the autonomous vehicles domain, where the simplifying assumption of rigid motion and capital resources of well funded corporations make labeling at scale tractable, several real world, lidar based scene flow datasets have been produced by using the tracks of the amodal object bounding boxes across a sequence of observations to produce per-point motion labels~\citep{caesar2020nuscenes, argoverse2,waymoopen, chodosh2023}. Of note, even with these simplifying assumptions, this labeling process is still extremely expensive --- as we discuss in \cite{vedder2024zeroflow} based on discussions with industry insiders we estimate it cost \$750,000 to label the 750 fifteen second sequences of the Argoverse 2 train split~\citep{argoverse2}.
In the autonomous vehicle domain, which typically assumes rigid motion, this allows human labelers to simply track the same amodal object bounding boxes they would use for object detection across a sequence of observations to produce flow estimates on a per-point basis~\citep{caesar2020nuscenes, argoverse2,waymoopen, chodosh2023}.

\subsection{What is Point / Particle Tracking and why is it hard?}

Point tracking is like optical flow, but sparse and over many image observations~\citep{sand2008particle}. Popular in applications like visual SLAM front-ends, classical approaches like SIFT \citep{sift}, SURF \citep{surf}, or ORB \citep{orb} use hand-built feature extractors; however, these approaches are brittle and require downstream applications like SLAM backends to handle their many failure cases. %Adjacent problems like semantic keypoint tracking focus on tracking a small number of semantically meaningful keypoints e.g.\ joint points on humans~\citep{ramanan2005strike, tompson2014real}

Modern, learning based approaches exhibit better general performance. Many approaches train on synthetic datasets like TAP-Vid-Kubric~\citep{tapvid}, per-frame feature extraction and then perform trajectory optimization~\citep{harley2022particle, doersch2022tapvid, karaev2023cotracker}. Notably, OmniMotion~\citep{wang2023omnimotion} takes a significantly different approach, instead performing test-time optimization to model the scene using per-frame neural radiance style reconstruction losses and a learned bijective mapping from a local coordinate frame into a shared global coordinate frame.



SEE https://openreview.net/pdf?id=Zmosb2KfzYd for related work

- trained feature extractors on synthetic data (PIPS https://arxiv.org/pdf/2204.04153)
- https://tapvid.github.io/

new datasets
 - 2d synethetic dataset generator https://github.com/google-research/kubric


recent work in 3D

 - dataset https://tapvid3d.github.io/


% Like with optical flow, scene flow 

%NATES PHD THESIS 3.2 % https://www.ri.cmu.edu/app/uploads/2024/08/nchodosh_phd_ri_2024.pdf#page=13.13


%instead of estimating motion vectors in the image plane, methods estimate motion in a 3D volume. For images, a major challenge comes from the lack of depth information, resulting in non-unique solutions in the general case~\citep{vedula1999}. which can be addressed with rigidity assumptions~\citep{teed2021raft3d}

%optical expansion~\citep{opticalexpansion}


motion description is not (yet) trivially solvable with the same recipes used to build our high quality, single frame methods; motion description is fundamentally association of structure between observations, and figuring out how to extract this from observational data without the need from extraordinarily expensive human annotations is currently an open research problem.

In this line of work, we try to address this problem through the lense of scene flow


% Thankfully, it is a beautiful time to be alive --- computer vision researchers have made great strides, first by kicking off the deep learning revolution with AlexNet's stunning results on ImageNet competition

focuses on understanding structure --- classification, object detection, semantic segmentation

Imagine you are driving your car down the highway, and something falls out of the back of a truck and into your lane; alternatively, you are in the kitchen, open the upper cupboard door, and a plate falls off a shelf, headed for your foot.  In these examples, recognizing, understanding, and then reacting to the motion of an unknown object is \emph{required} to avoid catastrophe. This makes high quality motion description a worthy problem for Computer Vision.

To humans, understanding motion is so ingrained in us that at first blush it is difficult to imagine why this is even a challenge --- we can look at an RGB video, which itself is just a series of 2D static observations of geometric structure, and intuitively piece together a 3D dynamic picture of objects, how they are moving, and even reliably predict where they will be at modest future time intervals.


you are not first doing object detection and then using a tracker to estimate motion to then act --- recognizing motion itself, regardless of object 




understanding frozen structure 

It does not take high minded academic philosophizing to recognize that  understanding motion is a critical part critical to understanding the physical world --- 

even the seemingly mundane daily task of driving a car requires a highly robust understanding of the motion of other objects (cars, pedestrians, dogs, debris, or even toddlers running to the ice cream truck). However, compared to understanding structure in static scenes (e.g.\ images or lidar point cloud sweeps), motion description has received relatively little attention


from catching a plate that falls as you open your cupboard door to dodging a trash can blowing , these 

dynamic tasks require robust perception of object motion as a bedrock to then effectively act.

%Understanding motion is prima facie important to understanding the world; 

%Much work in computer vision has been devoted to understanding the world's geometric structure, with enormous progress on 2D~\citep{alexnet} and 3D object detection~\citep{Peri_2022_CVPR,peri2022futuredet,peri2022towards,peri2023empirical}, but it's no less important to understand how that structure \emph{changes} with time.


%space constantly changes as we hurdle through time, and understanding how structure changes over time is just as fundamental as understanding the structure itself. However, throughout the history of computer vision, most attention has been given to understanding structure at a position Frozen in Time, with detectors and segmenters...

% Computer Vision as a field set out to build computer systems that understand the physical world. It 

%At its core, Computer Vision as a field aims to build computer systems that understand the world around them, enabling diverse downstream applications from advanced image editing tools to straight out of science fiction systems that hold fluent, natural language conversations with users about in-the-wild images~\citep{vlmsurvey} and generate arbitrary images~\citep{ImgEditing}.

%But, more fundamentally, 

% \section{Why has my PhD focused on Scene Flow?}

% My research has focused on describing and learning the \emph{dynamics} of the 3D world through the problem of Scene Flow. I strongly believe in The Bitter Lesson~\citep{bitterlesson}, but to me it's clear that general embodied AI systems need a deep intuition for the 3D world to be robust and sample efficient. My focus on describing dynamics was driven by the lack of scalable, data-driven methods at the time to learn this; while we have self-supervised problem of next frame prediction to get structure, when I started there were no unsupervised, data-driven methods to learn motion, and I felt this was a critical gap.

\section{How has my work contributed to motion understanding?}

\subsection{ZeroFlow: Scalable Scene Flow via Distillation}

We need \emph{scalable} Scene Flow methods, i.e.\ methods that improve by adding more raw data and more parameters. When I started this project, scene flow methods were either feed-forward supervised methods using human annotations (or from the synthetic dataset generator), or they were very expensive optimization methods. Worse, almost all of these methods did not run on full-size point clouds; they would downsample the point cloud to 8,196 points instead of the 50,000+ points in the (ground removed!) full point clouds. This is a \emph{critical} limitation, as it meant they are fundamentally unsuitable to detecting motion on all but the largest objects. This left us with only a couple optimization and feed-forward baseline scene flow methods that even tried to seriously solve the full scene flow problem.

ZeroFlow is a very simple idea: distill one of the few (very) expensive optimization methods (Neural Scene Flow Prior~\citep{nsfp}) into one of the few feed-forward networks that could handle full-size point clouds (FastFlow3D~\citep{scalablesceneflow}). This was far more successful than we expected, and ZeroFlow was state-of-the-art on the Argoverse 2 Self-Supervised Scene Flow Leaderboard (beating out the optimization teacher!). It was also 1000x faster than the best optimization methods, and 1000x cheaper to train than the human supervised methods.

While conceptually simple, ZeroFlow had several important take-home messages:

\begin{itemize}
    \item We have a working blueprint for scaling a scene flow method with data and compute
    \item At data scale, feed-forward networks will ignore uncorrelated noise in teacher pseudo-labels, enabling them to outperform the teacher
    \item With sufficient data scale, pseudolabel trained feed-forward networks can outperform human supervised methods with the exact same architecture
\end{itemize}


\subsection{\emph{I Can't Believe It's Not Scene Flow!}}

After publishing ZeroFlow, we spent a long time looking at visualizations of its flow results to get a deeper understanding of its shortcomings. We realized it (and all of the baselines) systematically failed to describe most small object motion (e.g. Pedestrians). Worse, we didn't know about these systematic failures using the standard metrics because, by construction, small objects have a very small fraction of the total points in a point cloud, and so their error contribution was reduced to a rounding error compared to large objects.

In order to properly quantify this failure, we proposed a new metric, \emph{Bucket Normalized Scene Flow}, that reported error per class, and normalized these errors by point speed to report a \emph{percentage} of motion described --- it's clear that 0.5m/s error on a 0.5m/s walking pedestrian is far worse than 0.6m/s error on a 25m/s driving car.

To show that this wasn't an impossible gap to close, we proposed a very simple and crude supervised baseline, \emph{TrackFlow}, constructed by running an off-the-shelf 3D detector on each point cloud and then associating boxes across frames with a 3D Kalman filter to produce flow. Despite the crude construction without any scene flow specific training, it was state-of-the-art by a slim margin on the old metrics but by an enormous margin on our new metric; it was the first method to describe more than 50\% of pedestrian motion correctly (hence the name, \emph{I Can't Believe It's Not Scene Flow!}).

The key take-home messages were:

\begin{itemize}
    \item There is a huge performance gap to close between prior art and a qualitative notion of reasonable flow quality
    \item Standard metrics were \emph{broken}, hiding this large gap
    \item This gap is closable, even with very simple methods, if we can properly measure it
\end{itemize} 

\subsection{Argoverse 2 2024 Scene Flow Challenge}

In order to push the field to close this gap, we hosted the \emph{Argoverse 2 2024 Scene Flow Challenge} as part of the CVPR 2024 \emph{Workshop on Autonomous Driving}. The goal was to minimize the mean normalized dynamic error of our new metric \emph{Bucket Normalized Scene Flow}, and featured both a supervised and an unsupervised track. The most surprising result was the winning supervised method Flow4D~\citep{flow4d} was able to \emph{halve} the error compared to the next best method, our baseline TrackFlow, and it did so with a novel feed forward architecture that was better able to learn general 3D motion cues, while using no additional fancy training tricks like class rebalancing.

Our key take-home message was that feed-forward architecture choice was a critically underexplored aspect of scene flow, and ZeroFlow and other prior work clearly suffered from inferior network design.

\subsection{Scene Flow as a Partial Differential Equation}

Under our new metric from \emph{I Can't Believe It's Not Scene Flow!}, it became clear that ZeroFlow's poor performance was at least partially inherited from the systematic limitations of its teacher. This motivated the need for a high-quality offline optimization method that, even if expensive, could describe the motion of small objects well.

To do this, we proposed \emph{EulerFlow}, a simple, unsupervised test-time optimization method that fits a neural flow volume to the \emph{entire} sequence of point clouds. This full sequence formulation, combined with multi-step optimization losses, results in extremely high quality unsupervised flow, allowing EulerFlow to capture state-of-the-art on the Argoverse 2 2024 Scene Flow Challenge leaderboard, beating out \emph{all} prior art, including all prior supervised methods. EulerFlow also displayed a number of emergent capabilities: it is able to extract long tail, small object motion such as birds flying, and it is able to do 3D point tracking across arbitrary time horizons for object using Euler integration.

The key take-home messages:

\begin{itemize}
    \item We now have a method to get extremely high quality unsupervised scene flow
    \begin{itemize}
        \item This is a prime candidate for a pseudolabel teacher
        \item This can be used to do long-tail object mining from motion cues
        \item This method works out-of-the-box on a wide variety of scenes, including indoor scenes
    \end{itemize}
    \item Multi-frame predictions were a critical factor to optimizing this representation; this likely has implications for loss design in feed-forward methods
\end{itemize}
 
\subsection{Artifacts and Code}

When I started, there were no model zoos and the open source codebases that were available were a mess. I sat down and wrote the ZeroFlow codebase from scratch, which then turned into SceneFlowZoo\footnote{\url{https://github.com/kylevedder/SceneFlowZoo}} with several other baseline implementations.

As part of \emph{I Can't Believe It's Not Scene Flow!} we also released a standalone dataloader and evaluation package which we used as the basis of the Argoverse 2 2024 Scene Flow Challenge. This codebase, BucketedSceneFlowEval\footnote{\url{https://github.com/kylevedder/BucketedSceneFlowEval}} is used by the model zoo, but is deep learning library agnostic (it produces everything in numpy arrays) and is thinly wrapped in the SceneFlowZoo codebase.

==> trackflow/abstract_hardstyle.tex <==
State-of-the-art scene flow methods broadly fail to describe the motion of small objects, and existing evaluation protocols hide this failure by averaging over many points. To address this limitation, we propose \emph{\oureval{}}, a new class-aware and speed-normalized evaluation protocol that better contextualizes error comparisons between object types that move at vastly different speeds. In addition, we propose \emph{\ourmethod{}}, a frustratingly simple supervised scene flow baseline that combines a high-quality 3D object detector (trained using standard class re-balancing techniques) with a simple Kalman filter-based tracker. Notably, \emph{\ourmethod{}} achieves state-of-the-art performance on existing metrics and shows large improvements over prior work on our proposed metric. Our results highlight that scene flow evaluation must be class and speed aware, and supervised scene flow methods must address point-level class imbalances. Our evaluation toolkit and code is available at \texttt{\url{https://github.com/kylevedder/BucketedSceneFlowEval}}.

%We make a startling observation: current scene flow methods consistently fail to describe motion on pedestrians and other small but important objects. We look into why this is surprising: current standard evaluation metrics hide this failure through averaging over many points, most of which come from large, common objects. We then present a new class-aware, speed normalized evaluation protocol (\emph{\oureval{}}) to quantify this failure. Finally, we present a frustratingly simple supervised scene flow baseline (\emph{\ourmethod{}}), built by bolting a high-quality pretrained detector (trained using many class rebalancing techniques) onto a simple tracker, that produces state-of-the-art performance on current standard evaluations and large improvements over prior art on our new evaluation. Ultimately, these findings make clear that all scene flow methods, supervised or unsupervised, must do class-aware evaluation, and supervised methods must do class-aware training.


%This method arbitrages work done on detectors to address class imbalance into scene flow, thereby addressing many problems with current methods and thus producing state-of-the-art performance on current standard evaluations, with large improvements over current methods on our new evaluation.

==> trackflow/abstract_old.tex <==
State-of-the-art scene flow methods consistently fail to capture the motion of smaller objects with fewer points (e.g.\ {\tt PEDESTRIANS} and {\tt WHEELED VRUs}). However, existing evaluation metrics fail to characterize this because average error is dominated by large objects (e.g.\ {\tt CAR} and {\tt OTHER VEHICLES}) which are responsible for most moving points. To address this limitation, we propose \emph{\oureval{}}, a new evaluation protocol that measures speed-normalized performance on a per-metaclass basis. Additionally, we present a frustratingly simple supervised scene flow baseline using an off-the-shelf pretrained detector and simple tracker that improves {\tt PEDESTRIANS} dynamic EPE by 20\% \neehar{Replace with exact number}. Our method, \emph{\ourmethod{}}, achieves state-of-the-art performance on standard evaluation protocols, and significantly outperforms prior work by over 10\% \neehar{Replace with exact number} on our improved metric.

==> trackflow/intro_hardstyle.tex <==
Scene flow estimation is the task of describing a 3D motion field between temporally successive point clouds~\cite{vedula1999, Zhai2020FlowMOT3M, baur2021slim, flownet3d, flowssl, scalablesceneflow, vedder2024zeroflow}. In theory, high quality flow estimators can provide a valuable signal about scene-level dynamics~\cite{scalablesceneflow, vedder2024zeroflow} 
%outside of a pretrained taxonomy 
for both online~\cite{Zhai2020FlowMOT3M} and offline~\cite{objectdetectionmotion} processing. Do state-of-the-art scene flow methods actually work well in practice? 

{\bf Status Quo.} Standard scene flow metrics suggest that existing methods can estimate motion to centimeter-level accuracy. %On Threeway EPE~\cite{chodosh2023}, a metric designed to separately measure static and dynamic performance, 
For example, ZeroFlow XL 5x~\cite{vedder2024zeroflow} achieves 
%state-of-the-art performance on the Argoverse 2 benchmark \cite{argoverse2}, featuring 
an average Threeway EPE~\cite{chodosh2023} of only 4.9 centimeters (1.9 inches) and a Dynamic EPE (averaged over points moving faster than 0.5 m/s)  of 11.7 centimeters (4.6 inches). Notably, these errors are relatively small compared to the scale of cars and pedestrians, implying that current scene flow methods produce high quality flow. On the scale of cars and people, these \emph{feel} like tiny errors and seem to imply that current scene flow methods are high quality.
%However, upon further investigation, we find that this is not the case! 

{\bf \oureval{}.}  We visualize flow predictions from several state-of-the-art supervised (FastFlow3D~\cite{scalablesceneflow}, DeFlow~\cite{zhang2024deflow}) and unsupervised (NSFP~\cite{nsfp}, ZeroFlow~\cite{vedder2024zeroflow}) approaches and find that all methods underestimate flow for small objects (\figref{teaserfigure}) with fewer lidar points (e.g. pedestrians and bicyclists). %Even on instances cherry picked to be \emph{easy} , existing methods describe larger objects well, but consistently fail to describe the motion of smaller objects with fewer lidar points (e.g. pedestrians and bicyclists). This is an alarming discovery. 
Surprisingly, existing scene flow metrics do not highlight such failure cases on these safety-critical categories because small objects only make up a tiny fraction of the dynamic points in a scene (\figref{fig:pointdistribution}).
%Existing scene flow metrics are failing to articulate this bad performance on these safety-critical objects because those objects are a tiny fraction of the (dynamic) points that make up a scene (\figref{fig:pointdistribution}). 
To address this limitation, we propose \emph{\oureval{}}, a new evaluation protocol that allows us to directly measure performance disparities across classes of different sizes and speed profiles. Specifically, \emph{\oureval{}} evaluates the \emph{percentage} of described motion, allowing us to normalize comparisons between objects moving at different speeds. 
% \begin{enumerate}
%     \item \todo{these two items are repeated verbatim in section 3} It's class aware. This allows us to call out performance on a per-class basis like detectors have done with \emph{mean Average Precision} for a decade~\cite{cocodataset}.
%     \item It's speed normalized on a per-point basis. This allows us to answer ``what percentage of object motion was described?'' by contextualizing against the speed of the object -- 0.5m/s of estimation error on a car moving 70 kph is negligible; 0.5m/s of estimation error on a pedestrian moving 0.5m/s is failing to describe all of the pedestrian's motion.
% \end{enumerate}
Our proposed evaluation metric takes inspiration from \emph{mean Average Precision} (mAP), a metric commonly used to evaluate object detectors. Notably, unlike existing scene flow metrics, mAP equally weights the performance of large common objects like cars and small rare objects like strollers. Therefore, state-of-the-art 3D object detectors use data augmentation and class re-balancing techniques~\cite{cbgs} to perform well on both common and rare classes. 
%With this in mind, we observe that supervised 3D lidar detectors are also evaluated on class-aware \emph{mean Average Precision}, and thus are engineered to perform well on smaller and rarer objects~\cite{cbgs}. 

{\bf \ourmethod{}.} Based on this observation, we propose \ourmethod{}, a frustratingly simple baseline that generates scene flow estimates using rigid transformations to describe point-level motion within a 3D object track.  Specifically, we run a state-of-the-art 3D object detector~\cite{wang2023le3de2e} followed by a simple 3D Kalman filter-based tracker~\cite{Weng2020_AB3DMOT} to generate object trajectories. %running a state-of-the-art detector to propose object boxes~\cite{wang2023le3de2e} followed by a simple 3D Kalman Filter tracker~\cite{Weng2020_AB3DMOT} to describe their motion. 
Despite its simplicity,  \emph{\ourmethod{}} achieves state-of-the-art performance on the standard metric of Threeway EPE. Even more importantly, \ourmethod{} significantly outperforms prior art on our \oureval{}, reducing error by 10\% across all classes, and 20\% on pedestrians in particular. Importantly, our simple baseline's state-of-the-art performance is an indictment of existing supervised scene flow methods. We argue that utilizing (well established) class re-balancing techniques can improve performance on rare safety-critical categories in real-world datasets, and evaluating scene flow methods using class and speed-aware metrics more closely reflects real-world performance. %Lastly, we find that unsupervised scene flow methods are also biased against small objects and fail to capture their flow. %This also has implications for the evaluation of unsupervised scene flow methods, which have broadly ignored the concept of object class and focused strictly on object geometry; these too are biased against smaller objects and fail to properly capture their flow.

{\bf Contributions}. We present three primary contributions.
\begin{enumerate}
  \item We highlight the qualitative failure of state-of-the-art scene flow methods on safety-critical categories like pedestrians and bicycles.
  \item We introduce \emph{\oureval{}}, a new evaluation protocol that allows us to quantify this qualitative failure on small objects.
  \item We propose \emph{\ourmethod{}}, a frustratingly simple baseline that achieves state-of-the-art performance on the standard metric of Threeway EPE. Additionally, it significantly outperforms prior art on our class-aware \emph{\oureval{}} metric.
\end{enumerate}


==> trackflow/intro_old.tex <==
The goal of scene flow estimation is to describe a 3D motion field between temporally successive point clouds~\cite{objectdetectionmotion, Zhai2020FlowMOT3M, baur2021slim, flownet3d, flowssl, scalablesceneflow, vedder2024zeroflow}. Robust scene flow estimators %stand to be enormously valuable across embodied computer vision domains by providing 
provide a valuable signal about the dynamics of the real world~\cite{scalablesceneflow, vedder2024zeroflow} outside of a pretrained taxonomy for offline~\cite{objectdetectionmotion} and online~\cite{Zhai2020FlowMOT3M} processing.

But where is scene flow \emph{today}? If we hope to detect motion from long tail, out-of-distribution objects, shouldn't we be able to robustly detect motion on common objects we \emph{already} know about? 
\neehar{I wouldn't start with these philosophical questions. I'd rather point to the existing metrics which suggest that "scene flow is solved"}

To qualitatively measure this, we run a collection of state-of-the-art  supervised (FastFlow3D~\cite{scalablesceneflow}, DeFlow~\cite{zhang2024deflow}) and unsupervised (NSFP~\cite{nsfp}, ZeroFlow~\cite{vedder2024zeroflow}) scene flow estimation methods on Argoverse 2~\cite{argoverse2}, an Autonomous Vehicle dataset. We cherry pick a scene (\figref{teaserfigure}) featuring two pedestrians walking close to the ego vehicle, producing unusually high density point clouds and thus making it a particularly easy instance to detect motion. Despite being picked to be easy, none of these state-of-the-art methods are able to describe meaningful motion. This is a surprising result, particularly in light of the fact that the supervised methods were human supervised on pedestrian motion directly, but it consistently holds across scenarios.

\neehar{Need to talk about why we think this is happening: Lower point density on some objects, all points are treated the same, doesn't really impact loss / optimization to ignore pedestrians / vulnerable road users.}

\neehar{Before jumping to what we do, we should frame it as "detector people have figured this out years ago w/ cbgs". Once we lay out that insight, then we need to transition to TracktorFlow}
To further illustrate this point, we present a frustratingly simple baseline, \emph{\ourmethod{}}, built using a high quality detector and a simple Kalman Filter-based tracker, that achieves state-of-the-art performance on Threeway EPE~\cite{chodosh2023}~(\sectionref{method}) and vastly superior performance on pedestrians and other vulnerable road users (\figref{teaserfigure}). However, this large performance gap is hidden by existing evaluation protocols; we analyze why, and then present a new evaluation protocol, \emph{\oureval{}}, that reveals performance across a variety of object categories (\sectionref{eval}), where \ourmethod{} quantitatively outperforms prior art by 10\% across all classes and up to 20\% on pedestrians. % a wide margin despite its simple nature. \neehar{Let's be more precise, 10\% on AV2, improving on Peds by 20\%.}


\neehar{We should end with some of the complaints we expect from a reviewer.}
\noindent Our primary contributions include:

%\neehar{First contribution is TracktorFlow, Second is Metric, Third is "extensive experiments", rule of threes.}
\begin{enumerate}
  \item A frustratingly simple Detector + Tracker scene flow method, \emph{\ourmethod{}} that achieves state-of-the-art performance on Threeway EPE~\cite{chodosh2023}
  \item A qualitative and quantitative evaluation of state-of-the-art scene flow methods, revealing very poor performance on smaller objects and, and the proposal of a new evaluation protocol, \emph{\oureval{}}, that quantifies this poor performance
  %\item Comprehensive experiments to ablate our design choices and demonstrate that our simple method achieves state-of-the-art results on the Argoverse 2 Scene Flow benchmark.
\end{enumerate}

==> trackflow/intro_thesis.tex <==
In \chapterref{zeroflow} we presented ZeroFlow, a training pipeline that achieved state-of-the-art performance on \emph{Threeway EPE}, a commonly used scene flow evaluation protocol developed by \cite{chodosh2023}. In this work, we start by asking a simple question: what does ZeroFlow's scene flow look like when we visualize it? What about other strong methods?

{\bf Status Quo.} Standard scene flow metrics suggest that existing methods can estimate motion to centimeter-level accuracy. %On Threeway EPE~\cite{chodosh2023}, a metric designed to separately measure static and dynamic performance, 
For example, ZeroFlow XL 5x~\cite{vedder2024zeroflow} achieves 
%state-of-the-art performance on the Argoverse 2 benchmark \cite{argoverse2}, featuring 
an average Threeway EPE~\cite{chodosh2023} of only 4.9 centimeters (1.9 inches) and a Dynamic EPE (averaged over points moving faster than 0.5 m/s)  of 11.7 centimeters (4.6 inches). Notably, these errors are relatively small compared to the scale of cars and pedestrians, implying that current scene flow methods produce high quality flow. On the scale of cars and people, these \emph{feel} like tiny errors and seem to imply that current scene flow methods are high quality.
%However, upon further investigation, we find that this is not the case! 

{\bf \oureval{}.}  We visualize flow predictions from several state-of-the-art supervised (FastFlow3D~\cite{scalablesceneflow}, DeFlow~\cite{zhang2024deflow}) and unsupervised (NSFP~\cite{nsfp}, ZeroFlow~\cite{vedder2024zeroflow}) approaches and find that all methods underestimate flow for small objects (\figref{teaserfigure}) with fewer lidar points (e.g. pedestrians and bicyclists). %Even on instances cherry picked to be \emph{easy} , existing methods describe larger objects well, but consistently fail to describe the motion of smaller objects with fewer lidar points (e.g. pedestrians and bicyclists). This is an alarming discovery. 
Surprisingly, existing scene flow metrics do not highlight such failure cases on these safety-critical categories because small objects only make up a tiny fraction of the dynamic points in a scene (\figref{fig:pointdistribution}).
%Existing scene flow metrics are failing to articulate this bad performance on these safety-critical objects because those objects are a tiny fraction of the (dynamic) points that make up a scene (\figref{fig:pointdistribution}). 
To address this limitation, we propose \emph{\oureval{}}, a new evaluation protocol that allows us to directly measure performance disparities across classes of different sizes and speed profiles. Specifically, \emph{\oureval{}} evaluates the \emph{percentage} of described motion, allowing us to normalize comparisons between objects moving at different speeds. 
% \begin{enumerate}
%     \item \todo{these two items are repeated verbatim in section 3} It's class aware. This allows us to call out performance on a per-class basis like detectors have done with \emph{mean Average Precision} for a decade~\cite{cocodataset}.
%     \item It's speed normalized on a per-point basis. This allows us to answer ``what percentage of object motion was described?'' by contextualizing against the speed of the object -- 0.5m/s of estimation error on a car moving 70 kph is negligible; 0.5m/s of estimation error on a pedestrian moving 0.5m/s is failing to describe all of the pedestrian's motion.
% \end{enumerate}
Our proposed evaluation metric takes inspiration from \emph{mean Average Precision} (mAP), a metric commonly used to evaluate object detectors. Notably, unlike existing scene flow metrics, mAP equally weights the performance of large common objects like cars and small rare objects like strollers. Therefore, state-of-the-art 3D object detectors use data augmentation and class re-balancing techniques~\cite{cbgs} to perform well on both common and rare classes. 
%With this in mind, we observe that supervised 3D lidar detectors are also evaluated on class-aware \emph{mean Average Precision}, and thus are engineered to perform well on smaller and rarer objects~\cite{cbgs}. 

{\bf \ourmethod{}.} Based on this observation, we propose \ourmethod{}, a frustratingly simple baseline that generates scene flow estimates using rigid transformations to describe point-level motion within a 3D object track.  Specifically, we run a state-of-the-art 3D object detector~\cite{wang2023le3de2e} followed by a simple 3D Kalman filter-based tracker~\cite{Weng2020_AB3DMOT} to generate object trajectories. %running a state-of-the-art detector to propose object boxes~\cite{wang2023le3de2e} followed by a simple 3D Kalman Filter tracker~\cite{Weng2020_AB3DMOT} to describe their motion. 
Despite its simplicity,  \emph{\ourmethod{}} achieves state-of-the-art performance on the standard metric of Threeway EPE. Even more importantly, \ourmethod{} significantly outperforms prior art on our \oureval{}, reducing error by 10\% across all classes, and 20\% on pedestrians in particular. Importantly, our simple baseline's state-of-the-art performance is an indictment of existing supervised scene flow methods. We argue that utilizing (well established) class re-balancing techniques can improve performance on rare safety-critical categories in real-world datasets, and evaluating scene flow methods using class and speed-aware metrics more closely reflects real-world performance. %Lastly, we find that unsupervised scene flow methods are also biased against small objects and fail to capture their flow. %This also has implications for the evaluation of unsupervised scene flow methods, which have broadly ignored the concept of object class and focused strictly on object geometry; these too are biased against smaller objects and fail to properly capture their flow.

{\bf Contributions}. In this chapter we present three primary contributions.
\begin{enumerate}
  \item We highlight the qualitative failure of state-of-the-art scene flow methods on safety-critical categories like pedestrians and bicycles.
  \item We introduce \emph{\oureval{}}, a new evaluation protocol that allows us to quantify this qualitative failure on small objects.
  \item We propose \emph{\ourmethod{}}, a frustratingly simple baseline that achieves state-of-the-art performance on the standard metric of Threeway EPE. Additionally, it significantly outperforms prior art on our class-aware \emph{\oureval{}} metric.
\end{enumerate}


==> zeroflow/perf_tables/argo.tex <==
\begin{tabular}{lrr|r|rrrr}
 \toprule
 & \multicolumn{2}{c|}{Runtime (ms)} & Point Cloud     & Threeway & Dynamic & Static & Static\\
 & &                                 & Subsampled Size & EPE      & FG EPE  & FG EPE & BG EPE\\ \midrule
 \humanlabels{FastFlow3D}*~\citep{scalablesceneflow} & \multirow{3}{*}{${29.33\pm}$} & \multirow{3}{*}{${2.38}$} & Full Point Cloud & 0.071 & 0.186 & 0.021 & 0.006 \\
 \ourmethodonex{}* (Ours) & & & Full Point Cloud & 0.088 & 0.231 & 0.022 & 0.011 \\
  \ourmethodthreex{} (Ours) & & & Full Point Cloud & 0.064 & 0.164 & 0.017 & 0.011  \\
  \ourmethodfivex{} (Ours) & & & Full Point Cloud & \textbf{0.056} & 0.140 & 0.017 & 0.011  \\ \midrule
  \humanlabels{FastFlow3D XL}  & \multirow{3}{*}{${260.61\pm}$} & \multirow{3}{*}{${1.21}$} & Full Point Cloud & 0.055 & 0.139 & 0.018 & 0.007 \\
  \ourmethodxlonex{} (Ours) & & & Full Point Cloud & 0.070 & 0.178 & 0.019 & 0.013 \\
  \ourmethodxlthreex{} (Ours) & & & Full Point Cloud & \textbf{0.054} & 0.131 & 0.018 & 0.012 \\
 NSFP w/ Motion Comp~\citep{nsfp} & $26,285.0\pm$ & $18,139.3$ & Full Point Cloud & 0.067 & 0.131 & 0.036 & 0.034  \\
 Chodosh et al.~\citep{chodosh2023} & $35,281.4\pm$ & $20,247.7$ & Full Point Cloud & 0.055 & 0.129 & 0.028 & 0.008 \\ \midrule
 Odometry & \multicolumn{2}{c|}{---} & Full Point Cloud & 0.198 & 0.583 & 0.010 & 0.000  \\
 ICP~\citep{chen1992object} & $523.11\pm$ & $169.34$ & Full Point Cloud & 0.204 & 0.557 & 0.025 & 0.028  \\
 \humanlabels{Gojcic}~\citep{gojcic2021weakly} & $6,087.87\pm$ & $1,690.56$ & $20000$ & 0.083 & 0.155 & 0.064 & 0.032  \\
 Sim2Real~\citep{jin2022deformation} & $99.35\pm$ & $13.88$ & $8192$ & 0.157 & 0.229 & 0.106 & 0.137  \\
 EgoFlow~\citep{tishchenko2020self} & $2,116.34\pm$ & $292.32$ & $8192$ & 0.205 & 0.447 & 0.079 & 0.090  \\
 PPWC~\citep{wu2020pointpwc} & $79.43\pm$ & $2.20$ & $8192$ & 0.130 & 0.168 & 0.092 & 0.129  \\
 FlowStep3D~\citep{kittenplon2021flowstep3d} & $687.54\pm$ & $3.13$ & $8192$ & 0.161 & 0.173 & 0.132 & 0.176  \\
 %Chodosh~\citep{chodosh2023} & $35281.4\pm$ & $20247.7$ & Full Point Cloud & 0.055 & 0.105 & 0.033 & 0.028 & 0.777 & 0.537 \\
 \bottomrule
\end{tabular}

==> zeroflow/perf_tables/waymo.tex <==
\begin{tabular}{lrr|r|rrrr}
 \toprule
 & \multicolumn{2}{c|}{Runtime (ms)} & Point Cloud     & Threeway & Dynamic & Static & Static\\
 & &                                 & Subsampled Size & EPE      & FG EPE  & FG EPE & BG EPE\\ \midrule
 \ourmethodonex{} (Ours) & \multirow{2}{*}{$21.66\pm$} & \multirow{2}{*}{$0.48$} & Full Point Cloud & 0.092 & 0.216 & 0.015 & 0.045 \\
 \humanlabels{FastFlow3D}~\citep{scalablesceneflow} & & & Full Point Cloud & 0.078 & 0.195 & 0.015 & 0.024 \\
 \midrule
 Chodosh~\citep{chodosh2023} & $93,752.3\pm$ & $76,786.1$ & Full Point Cloud & \textbf{0.041} & 0.073 & 0.013 & 0.039 \\
 NSFP~\cite{nsfp} & $90,999.1\pm$ & $74,034.9$ & Full Point Cloud & 0.100 & 0.171 & 0.022 & 0.108 \\
 ICP~\citep{chen1992object} & $302.70\pm$ & $157.61$ & Full Point Cloud & 0.192 & 0.498 & 0.022 & 0.055 \\
 \humanlabels{Gojcic}~\cite{gojcic2021weakly} & $501.69\pm$ & $54.63$ & 20000 & 0.059 & 0.107 & 0.045 & 0.025 \\
 EgoFlow~\citep{tishchenko2020self} & $893.68\pm$ & $86.55$ & 8192 & 0.183 & 0.390 & 0.069 & 0.089 \\
 Sim2Real~\citep{jin2022deformation} & $72.84\pm$ & $14.79$ & 8192 & 0.166 & 0.198 & 0.099 & 0.201 \\
 PPWC~\citep{wu2020pointpwc} & $101.43\pm$ & $5.48$ & 8192 & 0.132 & 0.180 & 0.075 & 0.142 \\
 FlowStep3D~\citep{kittenplon2021flowstep3d} & $872.02\pm$ & $6.24$ & 8192 & 0.169 & 0.152 & 0.123 & 0.232\\
 \bottomrule
 %Item,Mean (ms),Std (ms),Min (ms),Max (ms)
 %optimization,90999.1,74034.9,14309.1,349718
%refine,2753.16,2751.16,295.567,8254.49
\end{tabular}

==> zeroflow/tikz_figures/scene_flow_example.tex <==
\begin{tikzpicture}
    \setlength{\fboxsep}{0.0pt}
    \node[anchor=south west,inner sep=0] (image) at (0,0) {\fbox{\includegraphics[width=0.47\textwidth]{screenshot_figures/qualitative/argo/white_bg/gt_flow_cropped.png}}};
    \node[anchor=south west,inner sep=0] (image2) at (6.9,0) {\fbox{\includegraphics[width=0.47\textwidth]{screenshot_figures/qualitative/argo/white_bg/our_flow_cropped.png}}};
    \begin{scope}[x={(image.south east)},y={(image.north west)}]
      % Define the zoom area
      \coordinate (zoom_area_south_west) at (0.52,0.63);
      \coordinate (zoom_area_north_east) at (0.66,0.75);
      \coordinate (zoom_area_north_west) at (0.52,0.75);

      % Draw the zoom area rectangle
      \draw[black] (zoom_area_south_west) rectangle (zoom_area_north_east);

      % Draw the zoomed image
      \node[inner sep=0,right=-1.6cm of image, yshift=0.8cm] (zoomed_image) {{\fbox{\includegraphics[width=3.2cm]{screenshot_figures/qualitative/argo/white_bg/close_up_cropped_small.png}}}};

      % Draw the zoom lines
      \draw[black] (zoom_area_south_west) -- (zoomed_image.south west);
      \draw[black] (zoom_area_north_west) -- (zoomed_image.north west);
    \end{scope}
  \end{tikzpicture}
